The CAT Effect: Exploring the Impact of Casual Affective Triggers on Online Surveys' Response Rates

We explore the impact of Casual Affective Triggers (CAT) on response rates of online surveys. As CAT, we refer to objects that can be included in survey participation invitations and trigger participants' affect. The hypothesis is that participants who receive CAT-enriched invitations are more likely to respond to a survey. We conducted a study where the control condition received invitations without affective triggers, and the experimental condition received CAT-enriched invitations. We differentiated the triggers within the experimental condition: one-third of the population received a personalized invitation, one-third received a picture of the surveyor's cat, and one-third received both. We followed up with a survey to validate our findings. Our results suggest that CATs have a positive impact on response rates. We did not find CATs to induce response bias.

==> CAT CHI 2022/evaluation-partA.tex <==

\begin{table*}[h]
\begin{center}
\begin{tabular}{lccc}
\toprule 
   \textbf{Survey Element} & \textbf{Average Rating (SD)} & \textbf{Coeff} & \textbf{Std. Error} \\
   Realistic time estimate  & 4.01 (1.15)& 0.653$^{**}$& 0.28\\
   Investigator's information & 3.81 (1.21)& -0.186& 0.23\\
   Targeted audience scarcity& 3.78 (1.22) & 0.524$^{**}$& 0.23\\
   Personalized salutation  & 3.45 (1.19)& 0.02& 0.21\\
   Source of information & 3.36 (1.35)& 0.311& 0.19\\
   Attached picture  & 2.95 (1.42)& 0.957$^{***}$& 0.2\\
   
    \bottomrule
    \multicolumn{4}{l}{\scriptsize{$^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$, $^.p<0.1$}}
\end{tabular}
\end{center}
\caption{Average participation intentions on a 5-point Likert scale anchored between "strongly disagree" (1) and "strongly agree" (5) and regression coefficients and standard errors for participation intentions. The survey elements are sorted by their average rating, from highest to lowest.}
\label{tab:evalA}
\end{table*}

==> CAT CHI 2022/evaluation-partB.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{lccc}
\toprule 
    \textbf{} & \textbf{User Rating Average (SD)} &  \textbf{Coef OLR\_picture} & \textbf{Coef OLR\_participation} \\
   Pictures of Cats & 7.52 (1.72) & 0.788$^{***}$ & 0.375$^{***}$\\
   Pictures of Dogs & 7.25 (1.84)& -0.012& 0.196\\
   Pictures of Small Animals & 7.13 (1.68)& 0.125& 0.269\\
   
    \bottomrule
    \multicolumn{4}{l}{\scriptsize{$^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$, $^.p<0.1$}}
\end{tabular}
\end{center}
\caption{Average ratings for pictures of cats, dogs, and small animals on a scale from  "dislike extremely" (1) and "like extremely" (9) and regression coefficients among ratings of an attached picture as a survey invitation design element and participation intentions.}
\label{tab:evalB}
\end{table*}

==> CAT CHI 2022/inter-anova.tex <==

\begin{table}[h]
\begin{center}
\begin{tabular}{lccccccc}
\toprule 
\multicolumn{1}{c}{\textbf{Models}} & \multicolumn{7}{l}{Without Interaction: Response ~ CAT1 + CAT2 + (1 | reminder)} \\
\multicolumn{1}{c}{} & \multicolumn{7}{l}{With Interaction: Response ~ CAT1 + CAT2 + CAT1*CAT2 + (1 | reminder)} \\

    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
    \multicolumn{8}{c}{\textbf{Partial Participation}}\\
     \multicolumn{1}{c}{} & \multicolumn{1}{c}{npar} & \multicolumn{1}{c}{AIC} & \multicolumn{1}{c}{BIC} & \multicolumn{1}{c}{logLik} & \multicolumn{1}{c}{deviance}
    & \multicolumn{1}{c}{Chisq} & \multicolumn{1}{c}{Pr(>Chisq)} \\
Without Interaction  & 4  &  1508.1 & 1533.5 &  -750.03  & 1500.1  &  &  \\
With Interaction  & 5  &  1510.0 & 1541.8 &  -750.02  & 1500.0  &  0.0247 & 0.8752 \\

\multicolumn{8}{c}{\textbf{Complete Participation}}\\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
     \multicolumn{1}{c}{} & \multicolumn{1}{c}{npar} & \multicolumn{1}{c}{AIC} & \multicolumn{1}{c}{BIC} & \multicolumn{1}{c}{logLik} & \multicolumn{1}{c}{deviance}
    & \multicolumn{1}{c}{Chisq} & \multicolumn{1}{c}{Pr(>Chisq)} \\
Without Interaction  & 4  &  1228.1 & 1253.5 &  -610.05  & 1220.1  &  &  \\
With Interaction  & 5  &  1230.1 & 1261.8 &  -610.04  & 1220.1  &  0.0156 & 0.9006 \\

    \bottomrule
    \multicolumn{5}{l}{\scriptsize{$^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$, $^.p<0.1$}}
\end{tabular}
\end{center}
\caption{ANOVA comparisons for the regression models with and without interaction terms for partial participation and complete participation.}
\label{tab:anovamodels}
\end{table}

==> CAT CHI 2022/interaction-regression.tex <==

\begin{table*}[h]
\begin{center}
\begin{tabular}{lcccccc}
\toprule 
\multicolumn{1}{c}{\textbf{Random Effects}}& \multicolumn{3}{c}{\textbf{Partial Participation}} & \multicolumn{3}{c}{\textbf{Complete Participation}} \\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
    & \multicolumn{1}{c}{Variance} & \multicolumn{1}{c}{Std. Dev} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Variance} & \multicolumn{1}{c}{Std. Dev} & \multicolumn{1}{c}{}\\
Reminder(Intercept) & 3.373  &1.836  & 3.003  &  1.733     \\



   \multicolumn{1}{c}{\textbf{Fixed Effects}}& \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
    & \multicolumn{1}{c}{Coeffs} & \multicolumn{1}{c}{Std. Error} & \multicolumn{1}{c}{z-value} & \multicolumn{1}{c}{Coeffs} & \multicolumn{1}{c}{Std. Error} & \multicolumn{1}{c}{z-value} \\
    
    %\cmidrule(r){2-4} \cmidrule(l){5-7}
    Intercept  & -1.91  & 1.32 & -1.45 &-2.24 $^{.}$ & 1.25 & -1.8\\
    CAT1|1  & 0.54 $^{*}$ & 0.24 & 2.19 & 0.41 & 0.27 &  1.24 \\
    CAT2|1      & 0.31  & 0.27 & 1.16 &0.37  & 0.29& 1.48\\
    CAT1|1*CAT2|1 & 0.05 & 0.33 & 0.15 & -0.045  & 0.36& -0.12\\
  
    \bottomrule
    \multicolumn{5}{l}{\scriptsize{$^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$, $^.p<0.1$}}
\end{tabular}
\end{center}
\caption{Regression models for partial participation and complete participation that explored the interaction of affective triggers CAT1*CAT2 regarding response behavior. Email reminders were modeled as random effects.}
\label{tab:interact}
\end{table*}

==> CAT CHI 2022/partialregression.tex <==

\begin{table*}[h]
\begin{center}
\begin{tabular}{lcccccc}
\toprule 
\multicolumn{1}{c}{\textbf{Random Effects}}& \multicolumn{3}{c}{\textbf{Partial Participation}} & \multicolumn{3}{c}{\textbf{Complete Participation}} \\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
    & \multicolumn{1}{c}{Variance} & \multicolumn{1}{c}{Std. Dev} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Variance} & \multicolumn{1}{c}{Std. Dev} & \multicolumn{1}{c}{}\\
Reminder(Intercept)  & 3.001  &  1.732 &  &  3.375  &1.837  &   \\



   \multicolumn{1}{c}{\textbf{Fixed Effects}}& \multicolumn{3}{c}{} & \multicolumn{3}{c}{} \\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
    & \multicolumn{1}{c}{Coeffs} & \multicolumn{1}{c}{Std. Error} & \multicolumn{1}{c}{z-value} & \multicolumn{1}{c}{Coeffs} & \multicolumn{1}{c}{Std. Error} & \multicolumn{1}{c}{z-value} \\
    
    %\cmidrule(r){2-4} \cmidrule(l){5-7}
    Intercept  & -1.93  & 1.31 & -1.81 &-2.23 $^{.}$ & 1.23 & -1.47\\
    CAT1  & 0.57 $^{*}$ & 0.16 & 1.98 &0.38 $^{*}$ & 0.18 &  2.34 \\
    CAT2      & 0.35  $^{*}$ & 0.15 & 2.13 &0.34 $^{*}$  & 0.17& 3.51    \\
  
    \bottomrule
    \multicolumn{5}{l}{\scriptsize{$^{***}p<0.001$, $^{**}p<0.01$, $^*p<0.05$, $^.p<0.1$}}
\end{tabular}
\end{center}
\caption{Regression models for partial participation and complete participation that explored the impact of affective triggers (CAT1 and CAT2) on response behavior. Email reminders were modeled as a random effect.}
\label{tab:partialregr}
\end{table*}

==> CAT CHI 2022/partialresponses.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{L{2.5cm}lrrrlrr}
\toprule 
 & \multicolumn{1}{c}{\textbf{Control Condition}} & \multicolumn{3}{c}{\textbf{Experimental Condition}} & \multicolumn{3}{c}{\textbf{All Responses}}\\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
   & & \multicolumn{1}{l}{CAT1} & \multicolumn{1}{l}{CAT2} & \multicolumn{1}{l}{CAT1 and CAT2} \\
    %\cmidrule(r){2-4} \cmidrule(l){5-7}
    Before Reminders        &  17 (1.94\%) & 48 (3.89\%) & 26 (2.99\%) & 60 (4.78\%) & 151 (3.57\%)    \\
    After Reminders &  12 (1.39\%) & 17 (1.43\%) & 11 (1.3\%) & 38 (3.18\%) & 78 (1.91\%)   \\
    Total Responses  &  29 (3.31\%)& 65 (5.27\%)& 37 (4.25\%) & 98 (7.81\%) & 229 (5.41\%)  \\


    \bottomrule
    
\end{tabular}
\end{center}
\caption{Number of partial survey responses per condition before and after the reminder that was sent 14 days after the initial invitation. In parentheses, we provide the response rate per condition, that is, the percentage of partial responses per number of participants for each design group.}
\label{tab:partialresponses}
\end{table*}

==> CAT CHI 2022/responserates.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{L{2.5cm}lrrrlrr}
\toprule 
 & \multicolumn{1}{c}{\textbf{Control Condition}} & \multicolumn{3}{c}{\textbf{Experimental Condition}} & \multicolumn{3}{c}{\textbf{All Responses}}\\
    %& \multicolumn{3}{c}{\textit{Pseudo $R^2 = 10.2\%$}} & \multicolumn{3}{c}{\textit{$R^2 = 13.0\%$}} \\
    \addlinespace[0.1cm]
   & & \multicolumn{1}{c}{CAT1} & \multicolumn{1}{c}{CAT2} & \multicolumn{1}{c}{CAT1 and CAT2} \\
    %\cmidrule(r){2-4} \cmidrule(l){5-7}
    Before Reminders        &  13 (1.48\%) & 28 (2.27\%) & 23 (2.64\%) & 39 (3.11\%) & 103 (2.43\%)    \\
    After Reminders &  10 (1.16\%) & 19 (1.57\%) & 8 (0.94\%) & 31 (2.55\%) & 68 (1.65\%)   \\
    Total Responses  &  23 (2.63\%) & 47 (3.81\%) & 31 (3.56\%) & 70 (5.58\%) & 171 (4.04\%) \\


    \bottomrule
    
\end{tabular}
\end{center}
\caption{Number of complete survey responses per condition before and after the reminder that was sent 14 days after the initial invitation. In parentheses, we provide the response rate per condition, that is, the percentage of responses per number of participants for each design group.}
\label{tab:responserates}
\end{table*}

==> CAT CHI 2022/study.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{L{3cm}ccc}
\toprule 
     & \multicolumn{1}{c}{\textbf{CAT1 = 0}} & \multicolumn{1}{c}{\textbf{CAT1 = 1}} \\
    
    %\cmidrule(r){2-4} \cmidrule(l){5-7}
   \textbf{CAT2 = 0}& N = 875 & N = 1234   \\
    \textbf{CAT2 = 1} & N = 870 & N = 1254  \\
   
    \bottomrule
    
\end{tabular}
\end{center}
\caption{The 2x2 factorial study design that was implemented in this research}
\label{tab:study}
\end{table*}

==> CAT CHI 2022/survey-instrument.tex <==
% !TEX root = main.tex

\begin{table}[h]
\begin{center}
\begin{tabular}{|L{\linewidth}|}
\hline
\rowcolor{Gray}
Intention to participate, anchored between strongly disagree (1) and strongly agree (5) \\
\hline \\ [-2.2ex]
I would participate in the survey if I would receive an invitation that looks like this. \\
[0.8ex]
\hline
\rowcolor{Gray}
Perception of triggers, anchored between strongly disagree (1) and strongly agree (5) \\
\hline \\ [-2.2ex]
I would participate in this survey mainly because... \\
\tableIndent...it is only directed at the participants of this event.\\
\tableIndent...it explains where the surveyors obtained the information to contact me.\\
\tableIndent...it provides a realistic time estimate.\\
\tableIndent...it provides contact information of the investigator.\\
\tableIndent...if you read this please choose strongly disagree for this option.\\
\tableIndent...it is personalized.\\	\tableIndent...of the attached picture. \\
[0.8ex]
\hline
\rowcolor{Gray}
Perception of animal pictures, anchored between dislike extremely (1) and like extremely (9) (5)~\cite{peryam1957hedonic}\\
\hline \\ [-2.2ex]
Overall how much do you like or dislike... \\
\tableIndent...pictures of cats\\			
\tableIndent...pictures of dogs\\
\tableIndent...pictures of small animals\\
[0.8ex]
\hline
\rowcolor{Gray}
Demographics \\
\hline \\ [-2.2ex]
How old are you currently? (18 to 24, 25 to 34, 35 to 44, 45 to 54, 55 to 64, 65 to 74, 75 or older, Prefer not to say) \\
Are you...? (Female, Male, Non-binary, Prefer not to say) \\
Do you consider yourself a minority? (For example in terms of race, gender, expertise or in another way) (Yes, No, Prefer not to say) \\ [0.8ex]
\hline
\end{tabular}
\end{center}
\caption{Scales utilized for the validation survey}
\label{tab:app:instrument}
\vspace{-10pt}
\end{table}
